Code Vectors: Understanding Programs Through Embedded Abstracted Symbolic Traces

With the rise of machine learning, there is a great deal of interest in treating programs as data to be fed to learning algorithms. However, programs do not start off in a form that is immediately amenable to most off-the-shelf learning techniques. Instead, it is necessary to transform the program to a suitable representation before a learning technique can be applied. In this paper, we use abstractions of traces obtained from symbolic execution of a program as a representation for learning word embeddings. We trained a variety of word embeddings under hundreds of parameterizations, and evaluated each learned embedding on a suite of different tasks. In our evaluation, we obtain 93% top-1 accuracy on a benchmark consisting of over 19,000 API-usage analogies extracted from the Linux kernel. In addition, we show that embeddings learned from (mainly) semantic abstractions provide nearly triple the accuracy of those learned from (mainly) syntactic abstractions.

==> fig/overview.tex <==
%%% cSpell:disable

\begin{figure*}[!t]
\definecolor{artifactcolor}{RGB}{255,250,194}
\begin{tikzpicture}[
	node distance=0.5cm and 1cm,
    every node/.style={fill=white, font=\sffamily}, 
    align=center,
    base/.style={
    	rectangle, 
        rounded corners, 
        draw=black,
        minimum width=1cm,
        minimum height=1cm,
        text centered,
        font=\sffamily
    },
    artifact/.style={base, fill=artifactcolor},
    action/.style={base, fill=blue!30}
]
  \node (images)         [artifact                       ] {Docker\\Images};
  \node (transformer)    [action,   right= of images     ] {Transformer};
  \node (tsources)       [artifact, right= of transformer] {Transformed\\Sources};
  \node (merger)         [action,   right= of tsources   ] {Merger};
  \node (tracegen)       [action,   right= of merger     ] {Trace\\Generator};
  \node (abstractor)     [action,   right= of tracegen   ] {Abstractor};
  \node (abstractiondef) [artifact, above= of tracegen   ] {Abstraction\\Description};
  \node (atraces)        [artifact, right= of abstractor ] {Abstracted\\Traces};
  
  % --- 
  
  \draw[-{Latex[length=2mm]}] (images) -- (transformer);
  \draw[-{Latex[length=2mm]}] (transformer) -- (tsources);
  \draw[-{Latex[length=2mm]}] (tsources) -- (merger);
  \draw[-{Latex[length=2mm]}] (merger) -- (tracegen);
  \draw[-{Latex[length=2mm]}] (tracegen) -- (abstractor);
  \draw[-{Latex[length=2mm]},rounded corners=5pt] (abstractiondef) -| (abstractor);
  \draw[-{Latex[length=2mm]}] (abstractor) -- (atraces);
\end{tikzpicture}
\caption{Toolchain for converting programs (as Docker images) into abstracted
  traces.\label{Fi:Toolchain}}
\end{figure*}

%%% cSpell:ignoreRegExp /\\cverb\|.*?\|/
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper.tex"
%%% End: 

%  LocalWords:  artifactcolor RGB


==> fig/paths-histo.tex <==
\begin{figure}[tp]
  \begin{tikzpicture}
    \begin{axis}[
      title=Number of Paths in Ingested Procedures,
      width=0.82\linewidth,
      xbar,
      ymode=log,
      y=-0.2cm,
      bar width=0.3cm,
      enlarge x limits=0.005,
      axis y line*=left,
      axis line style=thick,
      % y axis line style = { opacity = 0 },
      axis x line       = none,
      ytick = {1,10,100,1000,10000,100000,1000000},
      ytick style={draw=none},
      y tick label as interval=false,
      yminorticks = false,
      yticklabels={%
        $\interval{1}{1}$,
        $\interval[open left]{1}{10}$,
        $\interval[open left]{10}{10^2}$,
        $\interval[open left]{10^2}{10^3}$,
        $\interval[open left]{10^3}{10^4}$,
        $\interval[open left]{10^4}{10^5}$,
        $\interval[open]{10^5}{\infty}$},
      nodes near coords,
    ]
    \addplot coordinates { 
      (90521,1) 
      (153931,10)
      (46336,100) 
      (11791,1000) 
      (4397,10000) 
      (1975,100000) 
      (2719,1000000)
    };
    \end{axis}
  \end{tikzpicture}
\caption{Approximately 98\% of ingested procedures have 5,000 or fewer paths.\label{Fi:PHISTO}}
\end{figure}
 
%%% cSpell:ignoreRegExp /\\cverb\|.*?\|/
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper.tex"
%%% End: 


==> trace-generation.tex <==
\section{Trace Generation\label{Se:TraceGeneration}}

Our toolchain consists of two phases: transformation and trace generation. As
input, our toolchain expects a corpus of buildable C projects and a description
of the abstractions to use during trace generation. Docker is used to
encapsulate each project in our corpus and the steps required to build that
project. As output, our toolchain produces a set of abstracted symbolic traces
which can be fed as input to word vector learners such as word2vec, GloVe, and
FastText.

A key feature of our toolchain is the ability to do many steps in parallel
configurations. For example, the trace generator is run every time an invocation
of \cverb|gcc| occurs in a Docker container in our input corpus (this also has
the benefit of making our system build-tool agnostic). If the build system being
used to invoke \cverb|gcc| is running in a parallel configuration then so will
our trace generator.

\input{fig/paths-histo}
\input{fig/abstractions} 
% JJH - ^ trying to get this on the page after the above figure...

A secondary feature of our toolchain is a focus on performance over precision.
The trace generator itself does not perform feasibility checking. It also has no
model of memory. It is an open question, and outside the scope of this work, as
to the effects of things like feasibility checking and a more precise model of
memory on the utility of the learned vectors.

Given these features and tradeoffs we will now explain the four main processes
in our trace generation toolchain:

\begin{enumerate}
\item \textbf{Transformer:} our toolchain's first step is to translate every
procedure into an OCaml file that encodes the procedure's control flow graph,
expressions, types, and path-profiling information. As a pre-processing step we
unroll any loops once before encoding the control flow graph.

\item \textbf{Merger:} once we have transformed each procedure into a
corresponding OCaml file we begin to selectively merge files. To generate traces
each OCaml file will need to be compiled and, to achieve maximum use of
our server resources, it is prudent to run a smaller amount of larger jobs
instead of many short-lived ones. We take advantage of the path-profiling
information in this phase by attempting to balance the total number of paths in
any given merged file.

\item \textbf{Trace Generator:} at this point we begin a massively parallel
process in which each transformed file is mounted into a Docker container with
the rest of the trace generator pre-loaded. \cverb|ocamlopt| is then used to
compile the transformed file and the resulting native executable is run in the
container. This executable streams traces to standard out which are compressed
and streamed to a mounted output directory. The only limit to the parallelism in
this phase is the number of available threads/compute nodes to run the Docker
jobs on (and the number of merged files created in the previous step). 

One particularly unique aspect of the Trace Generator is its compatibility with
high-throughput computing. Given access to a large cluster of machines (capable
of running Docker containers) we can generate traces for extremely large
programs with relative ease.

\item \textbf{Abstractor:} the final part of our trace generation takes a trace
and pattern matches user defined abstractions against it. We need some level of
abstraction in our pipeline to avoid writing out sentences that are too
specific. As an example, we would like to avoid encoding local variable names,
temporaries, or any other highly specific information as it conveys little
meaning. Without some kind of canonicalization our traces would be ineffective
as the input to a learner. 

\end{enumerate}

We have leveraged this pipeline to ingest the Linux kernel in an ``all-yes''
configuration.\footnote{The kernel we used was checked out (from GitHub's
mirror) at the following commit:
\cverb|fd7cd061adcf5f7503515ba52b6a724642a839c8|} In this configuration we are
able to ingest \texttt{311,670} procedures.\footnote{ We ignore
\cverb|crypto/vmac.c/vhash_update| during trace generation due to its size.} Our
pipeline takes approximately four hours to create its corpus of traces in this
configuration. As part of the trace generation we limit the symbolic execution
to only explore 5,000 paths. The histogram presented in \figref{PHISTO} shows a
summary of the paths-per-procedure in our corpus. We choose 5,000 paths as our
budget since approximately 98\% of procedures have 5,000 paths or fewer.

Throughout the rest of the paper we will use the Linux kernel, in the
configuration described above, as our dataset. When we reference any corpus of
traces, regardless of the abstractions used to configure the trace generator, we
will always be referring to an artifact that is derived from the kernel in the
configuration given above. 

%%% cSpell:ignoreRegExp /\\cverb\|.*?\|/
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper.tex"
%%% End:

